Complete $CP$ Eigen-bases of Mesonic Chiral Lagrangian up to $p^8$-order

Chiral perturbation theory systematically describes the low energy dynamics of meson and baryons using nonlinear Nambu-Goldstone fields. Using the Young tensor technique, we construct the pure mesonic effective operators up to $p^8$-order, one-to-one corresponding to contact amplitudes with the on-shell Adler zero condition. The off-shell external sources, non-vanishing under equation-of-motion conditions, are also added to the operator bases. We also show the invariant tensor bases using the Young tableau is equivalent to the trace bases with Cayley-Hamilton relations. Separated into different $CP$ eigenstates, at $\mathcal{O}(p^8)$ we obtain the operator lists of the 567 $C$+$P$+ operators, 483 $C$+$P$- operators, 376 $C$-$P$+ operators, and 408 $C$-$P$- operators for $SU(2)$ case, while there are 1959 $C$+$P$+ operators, 1809 $C$+$P$- operators, 1520 $C$-$P$+ operators, and 1594 $C$-$P$- operators for $SU(3)$ case, consistent with results using the Hilbert series.

==> App.B.p4-test.tex <==
\subsection{$p^4$ order operator list of $SU(2)$}
% \subsection{$SU(2)$}
\begin{center}
    \begin{longtable}{|c|c|c|c|c|c|}
    \caption{$SU(2)$ $\mathcal{O}{(p^4)}$ operators} \\
    \hline
        &&$C+P+$&$C+P-$&$C-P+$&$C-P-$\\
        \hline
        Type
        &111
        &${\mathcal{O}^{++}}_i^{(4)}$
        &${\mathcal{O}^{+-}}_i^{(4)}$
        &${\mathcal{O}^{-+}}_i^{(4)}$
        &${\mathcal{O}^{--}}_i^{(4)}$\\
        \hline
        $f^2$
        &111
        &$\langle f_{+\mu\nu} f_{+}^{\mu\nu}\rangle$
        &$\langle f_+^{\mu\nu} f_+^{\rho\lambda}\rangle\epsilon_{\mu\nu\rho\lambda}$&$\langle f_+^{\mu\nu} f_-^{\rho\lambda}\rangle\epsilon_{\mu\nu\rho\lambda}$
        &$\langle f_{+\mu\nu} f_-^{\mu\nu}\rangle$\\
        &111
        &$\langle f_{-\mu\nu} f_{-}^{\mu\nu}\rangle$
        &$\langle f_-^{\mu\nu} f_-^{\rho\lambda}\rangle\epsilon_{\mu\nu\rho\lambda}$
        &
        &\\
        \hline 
        $fu^2$
        &111
        &$\langle u_{\mu}u_{\nu} f_{+}^{\mu\nu}\rangle$
        &$\langle f_+^{\mu\nu}u^\rho u^\lambda\rangle\epsilon_{\mu\nu\rho\lambda}$
        &$\langle f_-^{\mu\nu}u^\rho u^\lambda\rangle\epsilon_{\mu\nu\rho\lambda}$
        &$\langle u_{\mu}u_{\nu}f_{-}^{\mu \nu}\rangle$\\
        \hline
        $u^4$
        &111
        &$\langle u_{\mu}u_{\nu} \rangle  \langle u^{\mu}u^{\nu} \rangle$
        &
        &
        &\\
        &111
        &$\langle u_{\mu}u^{\mu} \rangle  \langle u_{\nu}u^{\nu} \rangle$
        &
        &
        &\\
        \hline
        $\Sigma u^2$
        &111
        &$\langle \Sigma_{+} \rangle  \langle u^{\mu}u_{\mu} \rangle$
        &$\langle \Sigma_{-} \rangle  \langle u^{\mu}u_{\mu} \rangle$ 
        &
        &\\
        \hline
        $\Sigma^2$
        &111
        &$\langle\Sigma_{-}\rangle^2$
        &$\langle\Sigma_{-} \Sigma_{+}\rangle$
        &
        &\\
        &111
        &$\langle\Sigma_{+}\rangle^2$
        &$\langle \Sigma_{-} \rangle \langle \Sigma_{+} \rangle$
        &
        &\\
        &111
        &$\langle\Sigma_{+} \Sigma_{+}\rangle$
        &
        &
        &\\
        &111
        &$\langle\Sigma_{-} \Sigma_{-}\rangle$
        &
        &
        &\\
        \hline   
    \end{longtable} 
\end{center}
